A Structure Preserving Scheme for the Kolmogorov-Fokker-Planck Equation

In this paper we introduce a numerical scheme which preserves the long time behavior of solutions to the Kolmogorov equation. The method presented is based on a self-similar change of variables technique to transform the Kolmogorov equation into a new form, such that the problem of designing structure preserving schemes, for the original equation, amounts to building a standard scheme for the transformed equation. We also present an analysis for the operator splitting technique for the self-similar method and numerical results for the described scheme.

==> DiscreteTime.tex <==
With the discretization in place for \eqref{eq:Kolmogorov}, \eqref{eq:Rotating} and
\eqref{eq:SelfSimilar} we can introduce the time discretization.
More precisely, we will use a $\theta$-method to compute the diffusive terms.

For instance, for the Kolmogorov in Lagrangian variables, \eqref{eq:Rotating}, we state:
Given the time step $\Delta t$ then the solution, at time $t^{n+1}$, to \eqref{eq:Rotating} is given by the following $\theta$-method:
\begin{center}Given $g^n_h$, find $g^{n+1}_h \in V^h$ such that\end{center}
\begin{equation}\label{eq:RotatingDiscrete}
  (g_h^{n+1}, \chi_h) + \Delta t\, \theta\, a_{t^{n+1}}(g_h^{n+1}, \chi_h)
  = (g_h^n, \chi_h) - \Delta t\, (1 - \theta)\, a_{t^n}(g_h^n,\chi_h)
  \quad \forall \chi_h \in V^h\, .
\end{equation}
Notice that, taking $\theta=1$ gives Implicit Euler, $\theta = 0$ Explicit Euler, and $\theta=0.5$ Crank-Nicholson.\\
While for \eqref{eq:Kolmogorov} and \eqref{eq:SelfSimilar}, we respectively take\\
$$(\varphi_h^1, \chi_h) + \Delta t\, \theta\, {a}_{0}(\varphi_h^1, \chi_h) = (f_h^n, \chi_h) - \Delta t\, (1 - \theta)\tilde{a}_{0}(f_h^n,\chi_h) \qquad \forall \chi_h \in V^h$$
in place of \eqref{eq:TSKolmogorovHeatPart} in \autoref{alg:TSKolmogorov}, and
$$(\varphi_h^1, \chi_h) + \Delta t\, \theta\, {a}_{1-e^{-(n+1)\Delta t}}(\varphi_h^1, \chi_h) = (\tg_h^n, \chi_h) - \Delta t\, (1 - \theta)\tilde{a}_{1-e^{-n\Delta t}}(\tg_h^n,\chi_h) \qquad \forall \chi_h \in V^h$$
in place of \eqref{eq:ReactionDiffusion} in \autoref{alg:SimilaritySplitting}.

